MeMOT: Multi-Object Tracking with Memory

We propose an online tracking algorithm that performs the object detection and data association under a common framework, capable of linking objects after a long time span. This is realized by preserving a large spatio-temporal memory to store the identity embeddings of the tracked objects, and by adaptively referencing and aggregating useful information from the memory as needed. Our model, called MeMOT, consists of three main modules that are all Transformer-based: 1) Hypothesis Generation that produce object proposals in the current video frame; 2) Memory Encoding that extracts the core information from the memory for each tracked object; and 3) Memory Decoding that solves the object detection and data association tasks simultaneously for multi-object tracking. When evaluated on widely adopted MOT benchmark datasets, MeMOT observes very competitive performance.

==> tables/extra_dataset.tex <==
\begin{table*}[]
    \centering
    \small
    \setlength\tabcolsep{4.5pt}
    \begin{tabular}{l|cccccc}
    \toprule[1.5pt]
        \textbf{} &\textbf{\makecell{MOT17}}~\cite{milan2016mot16} &\textbf{\makecell{MOT20}}~\cite{dendorfer2020mot20} & \textbf{JTA}~\cite{fabbri2018learning} & \textbf{\makecell{CH val}}~\cite{shao2018crowdhuman} & \textbf{\makecell{CH train}}~\cite{shao2018crowdhuman} & \textbf{Mix}\dag\\\hline
        \textbf{Number of Images} & 5.3k & 8.9k & 230.4k & 5k & 10k &44k \\\hline
         \multicolumn{7}{c}{\textbf{MOT16/17} \cite{milan2016mot16}} \\\hline\hline
         TubeTK \cite{pang2020tubetk}  & \checkmark & & \checkmark & & &  \\
         FairMOT \cite{zhang2020fair}  & \checkmark & & &\checkmark & \checkmark& \checkmark\\
         JDE \cite{wang2019towards} & \checkmark & & & & & \checkmark\\
         TransCenter \cite{xu2021transcenter} & \checkmark & & & & \checkmark & \\
         TransTrack \cite{sun2020transtrack} & \checkmark & & & & \checkmark & \\
         Tracktor++ \cite{bergmann2019tracking} & \checkmark & & & & & \\
         CTracker \cite{peng2020chained} & \checkmark & & & & & \\
          \rowcolor{gray!20} TrackFormer \cite{meinhardt2021trackformer} & \checkmark & & & & & \\
         \rowcolor{gray!20} MOTR \cite{zeng2021motr} & \checkmark & & &\checkmark & &\\
         \rowcolor{gray!20} \textbf{MeMOT} (ours) & \checkmark & & &\checkmark & & \\\hline
         \multicolumn{7}{c}{\textbf{MOT20} \cite{dendorfer2020mot20}} \\\hline\hline
        FairMOT \cite{zhang2020fair} & & \checkmark& & & \checkmark& \checkmark \\
        TransCenter \cite{xu2021transcenter} & & \checkmark & & & \checkmark &\\
        TransTrack \cite{sun2020transtrack}  & & \checkmark & & & \checkmark & \\
        \rowcolor{gray!20} \textbf{MeMOT} (ours)  & & \checkmark & & \checkmark& & \\
    \bottomrule[1.5pt]
    \end{tabular}
    \vspace{-1.5mm}
    \caption{Training data for competing methods and MeMOT. \dag: a mixed dataset containing CityPerson~\cite{zhang2017citypersons} (3k), ETH~\cite{ess2008mobile} (2k), CalTech~\cite{dollar2009pedestrian} (27k), CUHK-SYSU~\cite{xiao2016end} (11k), and PRW~\cite{zheng2017person} (6k). Grey background indicates that these methods work with an in-network association solver (IAS), and the white background are with post-network association solver (PAS).}
    \label{tab:extra_data}
    \vspace{2.5mm}
\end{table*}


==> tables/memory_table.tex <==
\begin{table}
\footnotesize
%\setlength\tabcolsep{5.0pt}
\begin{tabular}{cc|cccccc}
\toprule[1.5pt]
        \textbf{$T_s$} & \textbf{$T_l$} & \textbf{IDF1} & \textbf{MOTA} & \textbf{HOTA} & \textbf{IDsw} & \textbf{IDFN} & \textbf{IDFP} \\\hline
         3 & 24 & 74.06& 65.77& \textbf{60.17} & \textbf{70} & 4878 & \textbf{7463}\\\hline
        \multirow{5}{*}{3}& 20 &73.87&  64.92 & 59.71 & 75& 4836 & 7588\\
        & 10 & 72.55 & \textbf{66.33}& 59.40 & 88 & 5142 &7991\\
        & 5 & 69.62 & 60.74 & 57.09 & 100 & 5939 & 8508\\
        & 3 & 69.60 & 60.39 & 57.00 & 101 & 5903 & 8591\\\hline
        2 & \multirow{3}{*}{24} & 70.32& 61.57& 58.74& 93& \textbf{4365} & 8177\\
        4 & &\textbf{74.45} & 64.87& 60.06 & 73& 4755& 7523\\
        5 & &74.32 & 64.27 & 59.62& 73& 4620& 7712\\
        
\bottomrule[1.5pt]
    \end{tabular}
\caption{Comparisons on different length of short-term $T_s$ and long-term $T_l$ memory.}
\label{tab:ablation:memory_length}
\end{table}
